Searching for low-mass companions at small separations in transition disks with aperture masking interferometry

Transition disks have large central cavities that have been spatially resolved during recent years. Cavities and other substructures in circumstellar disks are often interpreted as signposts to massive companions. We aim to search for stellar and substellar companions in the central regions of transition disks. We want to determine if these disks might be circumbinary in their nature, similar to the HD 142527 system. We observed four systems, HD 100453, HD 100546, HD 135344 B, and PDS 70, with the sparse aperture masking mode of VLT/SPHERE. We extracted the complex visibilities and bispectra from the H2 and H3 imaging data. A binary model was fit to the closure phases to search for companions and estimate detection limits. For validation, we also analyzed four archival datasets of HD 142527 and inferred the orbital elements and atmospheric parameters of its low-mass stellar companion. We have not detected any significant point sources in the four observed systems. With a contrast sensitivity of $\approx$0.004, we can rule out stellar companions down to $\approx$2 au and partially explore the substellar regime at separations $\gtrsim$3-5 au. The analysis of HD 142527 B revealed that its projected orbit is aligned with dust features in the extended inner disk and that the orbit could be close to coplanar with the outer disk. Atmospheric modeling confirms the low-gravity and slightly reddened spectral appearance. The bulk parameters are in agreement with dynamical constraints and evolutionary tracks. In contrast to HD 142527, we find no evidence that a close-in stellar companion is responsible for the resolved disk features of HD 100453, HD 100546, HD 135344 B, and PDS 70. Instead, the formation of giant planets or even low-mass brown dwarfs could be shaping the innermost environment ($\lesssim$20 au) of these circumstellar disks, as is the case with the planetary system of PDS 70.

==> extra.tex <==
Which are the known circumbinary disks? HD\,142527, GG\,Tau, CS\,Cha, V4046 Sgr, HD\,98800\,B

\citet{salyk2009} studied transition disks with high-resolution $M$-band spectroscopy and suggested their are two classes: cleared and partially depleted, based on veiling, CO emission strength, and accretion rate. Those with cleared inner disks are consistent with a close stellar companion and formation by photoevaporation. Two of those systems, HD\,98800\,B and CoKu\,Tau/4, do indeed host a close-in stellar companion.

\citet{cieza2012} performed a systematic study of transition disks using various diagnostics and observables and found that 1 out of 31 objects that they studied showed signatures of being a circumbinary disk, instead of e.g. grain growth or giant planet formation.

\citet{monnier2008} reported the discovery of a circumbinary disk around the Herbig Ae/Be star V892\,Tau using interferometric imaging techniques. They inferred that the central cavity is about five times the size of the projected binary separation, consistent with tidal truncation theory.

\citet{juhasz2017} studied observational signatures from warped disks due to the presence of a binary companion on a misaligned orbit, causing surface brightness asymmetries in scattered light and non-Keplerian kinematics.

\citet{ragusa2020} showed that circumbinary disks for mass ratio of $q > 0.05$ always develop an eccentricity, which correlates linearly with the cavity size.

\citet{ragusa2017} showed with 3D hydronymical simulations and radiative transfer that the origin of rings, dust horseshoes, and other non-axisymmetric structures in transition disks can be explained by the presence of massive companion ($q \gtrsim 0.04$).

Since the simultaneous measurements with the two filters are correlated, the difference between the retrieved parameters provides an estimate of the systematic uncertainty that had not been accounted for in the likelihood function, even though the (co)variances had been inflated. This term was added in quadrature to the statistical uncertainty. We also included the uncertainty on the true north, $-1.75 \pm 0.08$~deg \citep{maire2016b}, in the error budget of the position angle. For the orbital analysis that follows in the next section, we adopted the mean position and uncertainties of the two filters as the astrometry of that epoch, since the values are not independent measurements.

